Robust and Resource-Efficient Quantum Circuit Approximation

We present QEst, a procedure to systematically generate approximations for quantum circuits to reduce their CNOT gate count. Our approach employs circuit partitioning for scalability with procedures to 1) reduce circuit length using approximate synthesis, 2) improve fidelity by running circuits that represent key samples in the approximation space, and 3) reason about approximation upper bound. Our evaluation results indicate that our approach of "dissimilar" approximations provides close fidelity to the original circuit. Overall, the results indicate that QEst can reduce CNOT gate count by 30-80% on ideal systems and decrease the impact of noise on existing and near-future quantum systems.

==> sections/background.tex <==
\section{Background and Motivation}
\label{sec:background}


\subsection{Quantum Programs}

The unit of information in quantum computing is the qubit. This is a two-level abstraction, whose state is represented by $\ket{\psi} = \alpha\ket{0} + \beta\ket{1}$, which is a superposition of the $\ket{0}$ and $\ket{1}$ states. When this qubit is measured, its superposition collapses and it can be measured in state $\ket{0}$ with probability $\norm{\alpha}^2$ and in state $\ket{1}$ with probability $\norm{\beta}^2$, such that $\norm{\alpha}^2 + \norm{\beta}^2 = 1$. Similarly, an $n$-qubit entangled quantum system can be represented as a superposition of $2^n$ states: $\ket{\psi} = \displaystyle\sum_{k=0}^{k=n-1}\alpha_k\ket{k}$, such that $\displaystyle\sum_{k=0}^{k=n-1}\norm{\alpha_k}^2 = 1$.


A quantum program, or transformation, is a procedure (or computation) that takes a system from an initial state into a final state, as prescribed by its developer. There are multiple formalism spaces in which we can reason about quantum program behavior: 1) process~\cite{Kitaev:2002} metrics; 2) quantum state ~\cite{gilchrist,breuer,Nielsen-2010} metrics; and 3) domain specific output metrics. 

First, at the fundamental level, each program is
represented by an unitary matrix $U$. For a $n$ qubit system in initial state $\ket{\psi}$, the effect of the program is computed as $U \ket{\psi}$, where is U is a $2^n\times2^n$ unitary matrix.
In the unitary representation space, two quantum programs can be compared for ``equivalence'' (or distinguishability) using matrix distances such as the Hilbert-Schimdt distance, defined as \red{\begin{equation} \label{eq:hsn}
   \langle U, U_s \rangle_{HS} = \Trace(U^{\dag} U_s)
\end{equation}} Intuitively, process metrics compare how alike are two mathematical representations of a computation, based solely on their structure.

Synthesis algorithms use norms  to assess the solution quality, and their goal is to minimize $\norm{U - U_S}$, where $U$ is the unitary that describes the transformation and $U_S$ is the computed solution. They choose an error threshold $\epsilon$ and use it for convergence, $\norm{U-U_S} \le \epsilon$. Early synthesis algorithms use the diamond norm, while more recent efforts~\cite{qaqc,HSnormsynth} use the Hilbert-Schmidt  inner product between the conjugate transpose of $U$ and $U_s$. This is motivated by its lower computational overhead.


Second, under Deutch's computational model, a quantum program can be represented as a circuit. In this case, comparing two quantum programs requires examining and reasoning about their output. Given two state vectors, there are multiple distances used to asses their similarity,  e.g Total Variational Distance (TVD) or Jensen-Shannon (JS) divergence. \red{For example TVD is defined as ...}

Third, in practice the output probability distribution of a quantum program is transformed by a user defined procedure into a domain specific ``classical'' answer.
This domain result provides yet another method for program comparison. 


 
\subsection{Approximations}

It is often the case where we want to perform a particular quantum operation $A$ and because of external constraints we end up performing an approximation $B$, where $B \ne A$. Deciding which algorithm has executed is often referred to as distinguishability and existing methods use process and quantum state metrics. Note that there is no good quantitative generic formal approach  to relate these metrics to the quality of the domain science output.

We are interested in building program approximations using process metrics. Given a program represented by $U$, an aproximation is given by  $U_A$, where $\norm{U-U_A} \le \epsilon$. Unfortunately, a good approximation in this space does not guarantee the same relationship when measuring in the output space: two close programs may produce unacceptably different output at the domain level. This lack of strong direct correlation between process and output distances in illustrated in Figure~\ref{fig:emd_vs_rmd}.

\subsection{Resource Efficient Approximations} The performance of a quantum program is determined by the ``number'' of gates in its circuit. Thus, approximations can lead to performance improvements. Existing approaches~\cite{sc,bca,meetmiddle} use synthesis as a generating procedure: an approximation is a partial solution close to the original program.  The heuristics used to build circuits in synthesis  depend  on the hardware target.
For NISQ devices, the primary goal is mimizing the number of noisy two-qubit (CNOT) gates and the program critical path. For fault-tolerant devices, a more
complex procedure is used to minimize two-qubit gates and hard to correct single qubit (e.g. T) gates. 


\begin{figure}[t]
    \centering
    \includegraphics[scale=0.42]{figures/real_grove_3_rome}
    \caption{Probability of correct results over CNOT count of approximate circuits for 3 qubit Grover’s Algorithm on IBM Rome. Red dot is reference depth-optimal circuit.}
    \label{fig:grov3}
  \end{figure}
  
The benefit of approximations is illustrated by recent work~\cite{sc}. Figure~\ref{fig:grov3} shows the behavior of short depth approximations of a three qubit Grover algorithm on the IBM Rome~\cite{qhub}  system.  These are generated by enumerating the partial solutions produced using the BQSKit~\cite{bqskit,qsearch} synthesis infrastrcture. First, note that circuits up to $2\times$ shorter can produce the same quality output. Second, given the high level of hardware noise, many short approximations have better output fidelity when examined from the domain viewpoint.



Despite their potential, not many procedures to generate resource efficient approximations exist. ~\cite{sc,bca}  describe generative procedures using synthesis for circuits of up to five qubits, but lack a good criteria for selecting a priori a good approximation in practice. ~\cite{meetmiddle} describes a more scalable direct synthesis algorithm, but the approach leads to very long circuits, sometimes by orders of magnitude when compared to state-of-the-art.  


\subsection{Synthesis as Generating Procedure}

\red{Our approach is enabled by bottom up resource optimal synthesis (nothing else works well). Works at small scale.
  Given a circuit I have a procedure for generating short depth approximations of its ``optimal'' implementation by enumerating the search space.
Question here is how sparse this space is and what is his population. Tirthak to provide and display some data for say 3/4 qubit circuits, one long, one short...
 Say it depends on how hard/quantum  the circuit is.}

\subsection{Goals}
scalable to 100, resource efficient, robust.

\subsection{Quantum Computing and NISQ Errors}

A general quantum bit (qubit) can be represented using the state $\ket{\psi} = \alpha\ket{0} + \beta\ket{1}$, which is a superposition of the $\ket{0}$ and $\ket{1}$ states. When this qubit is measured, its superposition collapses and it can be measured in state $\ket{0}$ with probability $\norm{\alpha}^2$ and in state $\ket{1}$ with probability $\norm{\beta}^2$, such that $\norm{\alpha}^2 + \norm{\beta}^2 = 1$. Similarly, an $n$-qubit entangled quantum system can be represented as a superposition of $2^n$ states: $\ket{\psi} = \displaystyle\sum_{k=0}^{k=n-1}\alpha_k\ket{k}$, such that $\displaystyle\sum_{k=0}^{k=n-1}\norm{\alpha_k}^2 = 1$. This property of quantum computing can be leveraged to speed up computation over classical systems, which can only represent one state at a time.

A quantum system can be put into a desired superposition state using quantum gates or operations. For example, a one-qubit NOT operation can be used to rotate the state of qubit ($\ket{0}$ to $\ket{1}$ or vice versa), while a two-qubit controlled-NOT or CNOT operation can be used to entangle two qubits and apply a NOT gate to the ``target'' qubit if the ``control'' qubit is in the $\ket{1}$ state. When these operations are applied in succession to one another, they form a ``quantum circuit'' that represents and executes the corresponding ``quantum algorithm.'' Note that all quantum algorithms can be represented as a sequence of one-qubit rotation gates and two-qubit CNOT gates.

However, existing quantum systems and projected near-term future quantum systems suffer from a pack of different types of errors. For instance, they are affected by state-preparation and measurement (SPAM) errors, which are errors related to preparing the state of the quantum system before computation and measuring the quantum state post computation. Another type are errors are related to the coherent errors related to applying one-qubit and two-qubit quantum operations to a qubit. These errors get compounded over the course of a quantum circuit, as a circuit runs many quantum operations. On existing quantum computers, two-qubit operation error rate tends to be an order of magnitude above one-qubit operation error rate. Lastly, qubits also suffer from decoherence, whereby their states suffer amplitude and phase degradation over time. Typically, qubits lose their coherence in the order of hundreds of microseconds after their state is prepared.

These errors make is difficult to run long quantum circuits with many two-qubit (CNOT) operations on existing and near-term quantum computers. Next, we discuss a method to reduce the total number of CNOT operations of a circuit and also reduce the circuit depth (circuit depth is measured as the number of CNOT operations on the critical path of a quantum circuit -- the critical path determines the time taken to run a quantum circuit).

% \subsection{Quantum Circuit Synthesis}

% Quantum circuit synthesis is the technique used to find a circuit for a quantum algorithm that is mathematically equivalent to the original algorithm circuit, but is less deep and has fewer CNOT operations. An $n$-qubit quantum algorithm can be represented as an $N\times N$ unitary matrix, where $N = 2^n$. This unitary matrix can be calculated by taking a product of all the operations run by quantum algorithm (note that all quantum operations can be represented using a unitary matrix. For example, if an algorithm runs $O$ operations one after another, and the $o^{th}$ operation is represented using the unitary $U_k$, the unitary of the entire algorithm can be calculated as $U = U_O U_{O-1}\dots U_2 U_1$.

% Quantum circuit synthesis is the process of finding an equivalent unitary $U'$ (obtained using a shorter circuit with fewer CNOT gates) for $U$, such that the ``distance'' between the two is minimized. This distance is referred to as the ``process distance.'' It is difficult to come up with an exact solution for an equivalent circuit for $U$ analytically, especially for circuits larger than two qubits~\cite{}. For this reason, previous works have proposed numerical optimization solutions~\cite{}. These works attempt to construct the synthesized circuit one layer at a time (a layer typically consists of a combination of one-qubit rotation gates and two-qubit CNOT gates). Once a layer is embedded onto the synthesized circuit, numerical optimization methods are used to optimize the rotation angles such that the process distance between the unitary of the synthesized circuit ($U'$) and the original (target) circuit ($U$) is minimized. If the distance is within a certain acceptable threshold, the solution is accepted. Typically, a variation of the Hilbert-Schmidt (HS) distance is used to calculate whether the process distance between $U'$ and $U$ is within the acceptable threshold of $\epsilon$: $1 - \frac{\norm{\text{tr}(U^\dagger U')}}{N} < \epsilon$ or $\sqrt{1 - \frac{\norm{\text{tr}(U^\dagger U')}^2}{N^2}} < \epsilon$. These metrics have a value between 0 and 1, with 0 being the best (lowest distance). The process distance needs to be calculated thousands of times during the numerical optimization process. The HS distance is used for this process because it computationally more efficient than other distance metrics such as the diamond norm~\cite{}.

% If an acceptable solution is not found, another layer of gates is added to the synthesized circuit and again the numerical optimization is performed. Note that every time a layer is added, the optimizer has increased degrees of freedom due to the more rotation angles, getting the synthesized circuit's unitary closer to the target circuit's unitary. For most circuits, synthesized circuit should have a lower depth and fewer CNOT gates before the acceptable threshold is reached. In fact, previous works have shown that an improvement of $50-100\%$ is also possible, depending on the algorithm~\cite{}. In this regard, the synthesis approach is promising to reduce the depth and number of CNOT operations of a circuit, which can greatly help decrease the errors faced by algorithms when run on NISQ devices.

% However, the synthesis technique is not scalable with increase in circuit size. This is because the unitary of the circuit scales exponentially with the number of qubits in the circuit. This makes the process of calculating the process distance during each iteration of numerical optimization exponentially slower with increase in circuit size. For example, a 10-qubit circuit requires $2^{10^2}$ inner products to calculate the process distance each time. In fact, it is difficult to calculate the target unitary of the entire circuit in the first place because it requires multiplying large quantum operation unitaries. Thus, it is infeasible to perform synthesis on a full circuit unitary for large circuits. Next, we look at solutions proposed to mitigate this problem.

% \begin{figure}[t]
%     \centering
%     \includegraphics[scale=0.42]{figures/partitioning_cartoon.pdf}
%     \caption{Example of partitioning a circuit (represented using partition unitaries $U_1$ and $U_2$) for synthesis. Isolated squares represent one-qubit rotation gates, squares connected to another qubit represent CNOT gates where the circle is the control qubit and the square is the target qubit, and the black squares at the end represent measurement gates. Operations are applied in order from left to right.}
%     \label{fig:part_cart}
% \end{figure}

% \subsection{Synthesis Scalability and Partitioning the Circuit for Synthesis}

% The solution to the problem of scaling the circuit synthesis approach is to partition the circuit into blocks of smaller sizes~\cite{}. Fig.~\ref{fig:part_cart} shows how this can be achieved for an example circuit of four qubits. Assuming that we can synthesize circuits that are up to three qubits in size (larger than three qubits is computationally infeasible in this example), if we partition the four-qubit circuit into two blocks of three-qubits, we can synthesize the two blocks separately to generate circuits equivalent to their corresponding unitaries: $U_1$ and $U_2$. All the operations under the yellow region can be combined to form the $U_1$ block and all the operations under the blue region can be combined to form the $U_2$ block. The blocks have to formed such that there are no connections (in terms of two-qubit CNOT operations) between the two blocks. Otherwise, they can be considered entangled and cannot be synthesized separately. QGo~\cite{}, a circuit partitioning approach, forms partitions by traversing the circuit left to right and creating $n$-qubit blocks that are as deep as possible in order to generate the fewest number of blocks and have the maximum reduction in depth post synthesis.

% In terms of our example circuit, the unitary $U_1$ can be synthesized such that $1 - \frac{\norm{\text{tr}(U^\dagger_1 U'_1)}}{N_1} < \epsilon_{1}$ and the matrix $U_2$ can be synthesized such that $1 - \frac{\norm{\text{tr}(U^\dagger_2 U'_2)}}{N_2} < \epsilon_{2}$. When the synthesized circuits are obtained for $U_1$ and $U_2$, they can be put together to form the full synthesized circuit. Note that this approach is scalable because we limit the block size to what is computationally acceptable. Synthesizing in this manner does not require generating the target unitary for the full circuit, nor does it require calculating the process distance for the entire circuit's unitary. However, this partitioning approach also has several limitations, which we discuss in the following section

% \subsection{The Distance Approximation Problem of Circuit Partitioning}

% While circuit partitioning makes synthesis scalable, the primary problem faced by previous works is that the distance cannot be directly controlled.

% \subsubsection{Bounding the Full Circuit Process Distance}

% Post partitioning the circuit, synthesis is performed for the individual blocks of the circuit. For each of the blocks, it can be ensured that the process distance of the block is within a certain threshold $\epsilon$. However, when all the synthesized blocks are put back together to form the full synthesized circuit, the process distance can exceed the threshold $\epsilon$. Previous partitioning work does not demonstrate how the process distance compounds (e.g., multiplicatively) when the blocks are combined to form the synthesized circuit. Without having a theoretical bound on the process distance of full circuit, the process distance thresholds of its blocks may have to kept unnecessarily small to be on the safe side. This means that the synthesized blocks likely end up being longer than they need to be as more layers are typically required during the numerical optimization process if the distance threshold is very small. This can result in sub-optimal synthesis performance with more depth and CNOT operations than there is a need for in order for the full circuit synthesized unitary to be mathematically equivalent to its target unitary. Overcoming this problem can help us synthesize shorter circuits with fewer CNOT operations. To mitigate this issue, we provide a theoretical proof (in Sec.~\ref{sec:solution}) to bound the full circuit process distance based on the process distances of its blocks without the need to directly calculate the process distance of the full circuit. 

% In addition to the bounding problem, another issue faced by synthesized circuits relates how the process distance translates to the circuit output, as discussed next.

% \begin{figure*}[t]
%     \centering
%     \subfloat[][10-Qubit TFIM]{\includegraphics[scale=0.65]{figures/tvd_vs_rmd_tfim_10.pdf}}
%     \subfloat[][9-Qubit SUP]{\includegraphics[scale=0.65]{figures/tvd_vs_rmd_sup_9.pdf}}
%     \subfloat[][9-Qubit ADDER]{\includegraphics[scale=0.65]{figures/tvd_vs_rmd_adder_9.pdf}}
%     \subfloat[][10-Qubit MUL]{\includegraphics[scale=0.65]{figures/tvd_vs_rmd_mul_10.pdf}}
%     \caption{Relationship between the process distances of different synthesized circuits and their corresponding output distances (TVD) for different algorithms. Note that both axes are in log scale. The results indicate an uncorrelated relationship between process distance and output distance.}
%     \label{fig:rmd_vs_tvd}
% \end{figure*}

% \subsubsection{Relationship of the Process Distance with the Output Distance}

% While the process distance of the circuit needs to be considered when performing synthesis, the ``output distance'' of the circuit comes into play when the output of the algorithm is measured for different algorithms. Note that the output distance cannot be used during synthesis due to the fact that the state of quantum system can only be represented using its unitary. Moreover, when the circuit is partitioned, each block cannot be optimized using an output distance metric because individual blocks have no output of their own. Only the full circuit has an output and the full circuit is only measured upon circuit completion. It can neither be measured in-between the circuit for different blocks, nor can the input of the blocks be determined to perform output distance metric calculation as it requires full circuit unitary simulation. Thus, the process distance must be used for synthesis. However, from the perspective of algorithm usability, the output is of the most importance. Therefore, it is important to determine how far the output of the synthesized circuit is from the output of the original circuit, i.e., what is their output distance.

% Depending on the requirement of the algorithm, the output distance can be measured in different ways. However, one universal measurement is the total variation distance or the TVD of the output. The TVD measures the difference in the probabilities of two probabilities distributions. Because the output of quantum program is probabilities, we can use the TVD to measure the difference between the output of the original circuit and the measured circuit. For an $n$-qubit circuit, which has $N=2^n$ output states, the TVD can be calculated as $\frac{1}{2}\sum_{k=1}^{k=N}\abs{p(k) - p'(k)}$, where $P(k)$ is the probability of state $k$ with the original circuit and $p'(k)$ is the probability of state $k$ with the synthesized circuit. TVD has a value between 0 and 1, with 0 being the best (lowest distance).

% While, in general, reducing the process distance also reduces the output distance, the correlation between the process distance and the output distance is not one-to-one. This is shown in Fig.~\ref{fig:rmd_vs_tvd}, which demonstrates the relationship between the process distances of different synthesized circuits and their corresponding output distances for a few algorithms. Evidently, the TVD does not necessarily increase/decrease with increase/decrease in process distance. Because it is not straightforward to calculate the process distance or the output distance for large quantum circuits, we cannot assume that simply selecting the circuit with a low process distance (based on the bound proved in that next section) will yield a low output distance. We have to select the synthesized circuits carefully in order to attain our two goals: (1) to reduce the circuit depth and number of CNOT gates sufficiently in order to decrease the impact of hardware and control errors in the NISQ era, and (2) to reduce the overall process distance and output distance without the ability to calculate them directly. In the following section, we present the solutions to these problems. 







==> sections/fidelity.tex <==
\section{Improving Output Quality}
\label{sec:avg}

\red{Still no correlation HS - TVD. One approx may not be enough. Introduce the idea of average. The question is how to sample uniformly. Approach inspired by the generating procedure but can be easily changed. Conjecture is that we need to choose many structurally different approximations. Need to  make sure we evaluate - vs 0.}

\red{\subsection{Approximations and Noise}. Add pictures with circles and splain some...}


\red{\subsection{Generating Procedure} Describe principles.}

\begin{figure*}[t]
    \centering
    \subfloat[][10-Qubit TFIM]{\includegraphics[scale=0.65]{figures/tvd_vs_rmd_tfim_10.pdf}}
    \subfloat[][9-Qubit SUP]{\includegraphics[scale=0.65]{figures/tvd_vs_rmd_sup_9.pdf}}
    \subfloat[][9-Qubit ADDER]{\includegraphics[scale=0.65]{figures/tvd_vs_rmd_adder_9.pdf}}
    \subfloat[][10-Qubit MUL]{\includegraphics[scale=0.65]{figures/tvd_vs_rmd_mul_10.pdf}}
    \caption{Relationship between the estimated process distance upper bound and the actual process distance for different algorithms. Note that both axes are in log scale. The results indicate a relatively tight bound across all algorithms.}
    \label{fig:emd_vs_rmd}
  \end{figure*}

  \subsection{Tightness of the Process Distance Upper Bound in Practice}

While the derivation of the upper bound is useful for practical purposes, it is important to establish whether the upper bound is tight in most cases. If the bound is not tight, i.e., the actual process distance tends to be much lower than the upper bound, then using the upper bound to perform synthesis might result in sub-optimal results (circuits with more depth and greater number of CNOT gates) because the synthesis numerical optimizer may need to meet unnecessarily high standards; it may need to satisfy a lower error threshold to keep the full circuit process distance upper bound low, while the actual full circuit process distance is in fact much lower. If the bound is relatively tighter, then it can be assumed the circuit depth required to keep the process distance lower than the upper bound is reasonable and not sub-optimal as the actual process distance should be close to the upper bound.

Unfortunately, the relationship between the derived process distance upper bound and the actual process distance cannot be directly/theoretically proven as it algorithm specific and varies depending on how the algorithm circuit is constructed and partitioned. Therefore, we demonstrate this relationship using real algorithm examples. Fig.~\ref{fig:emd_vs_rmd} shows the relationship between the estimated process distance upper bound and the actual process distance for different algorithms. The results indicate a relatively tight bound across all algorithms as both metrics (estimated process distance upper bound and the actual process distance) tend to be in the same order of magnitude. Therefore, we can safely use the theoretical process distance upper bound to generate circuits with short depths, while remaining mathematically equivalent to the original algorithm circuit.

\begin{figure}[t]
    \centering
    \includegraphics[scale=0.54]{figures/output_distance_cartoon.pdf}
    \caption{A visual example of how selecting multiple synthesized circuits can help lower the output distance: (a) shows the output distance vs. circuit depth relationship of multiple synthesized circuits, and (b) shows the average output distance if $M$ circuits with the lowest depth are selected.}
    \label{fig:out_dist_cart}
\end{figure}

==> sections/solution.tex <==
\section{Composing and Scalable Approximation Generation}
\label{sec:solution}


\red{For large circuits we can't use synthesis as a direct generator. Introduce the QGo approach, show picture of tiled circuit.
  This introduces the need for composition, our approach is enabled by theorem..}


In this section, we present \sol, a solution to the problem of approximating the process distance when partitioning and reducing the output distance. First, we present a theoretical upper bound on the process distance of the full circuit based on the process distances of the circuit partitions. Our theoretical derivation shows that the full circuit process distance can be effectively bounded simply by bounding the process distances of the smaller partitions, without the need to calculate it directly for the large circuit. Second, we show that this theoretical upper bound is relatively tight and is in the same order of magnitude as the actual full circuit process distance across different quantum algorithm circuits.

Third, we demonstrate that to effectively utilize the theoretical upper bound, \sol{} needs to be aware of the output distance as the output distance may not always be directly proportional to the process distance used for synthesis. To overcome this problem, finally, we present the design and implementation of \sol{}. \sol{} combines circuit partitions to form the full circuit in a manner that the full circuit process distance is bounded, the depth and number of CNOT operations in the circuit are reduced, and the output distance is minimized. It does so by leveraging the fact that several different combinations of partitions with low circuit sizes, each with a different output distance - process distance relationship can be obtained under the same process distance bound. These combinations of partitions can be used to reduce the circuit size, as well as reduce the output distance on average.

\subsection{Theoretical Process Distance Upper Bound}

We prove the theoretical upper bound for the example circuit shown in Fig.~\ref{fig:part_cart}. The proof can be derived for the circuit partitioned into two blocks without any loss of generality, and it can then be extended to a circuit partitioned into $K$ blocks.

We want the process distance of the unitary $U$ of the full circuit to be bounded without performing synthesis on the full circuit due to the lack of scalability: $\sqrt{1 - \frac{\norm{\text{tr}(U^\dagger U')}^2}{N^2}} < \epsilon$. $U$ is an $N \times N$ matrix, where $N$ is $2^n$, where $n$ is the number of qubits in the full circuit. We choose the $\sqrt{1 - \frac{\norm{\text{tr}(U^\dagger U')}^2}{N^2}}$ metric for process distance as it is a reasonable metric to measure unitary equivalency, it is computationally efficient, and it gives us the ability to prove a bound on it without directly calculating it, as we will see later in this section. The $\epsilon$ bound needs to be derived based on the process distances of its circuit blocks. Recall that the partitioned blocks are small enough to be efficiently synthesizable and therefore, have known process distances. The example circuit has two blocks and these blocks have the below two process distance bounds by construction (synthesis is performed in a manner that ensures that these bounds are met).
\begin{equation}
    \begin{gathered}
    \sqrt{1 - \frac{\norm{\text{tr}(U^\dagger_1 U'_1)}^2}{N_1^2}} \le \epsilon_{1} \ \ \ , \ \ \ 
    \sqrt{1 - \frac{\norm{\text{tr}(U^\dagger_2 U'_2)}^2}{N_2^2}} \le \epsilon_{2}
    \end{gathered}
    \label{eq:thames}
\end{equation}

Here, $N_1$ and $N_2$ are the dimensions of $U_1$ and $U_2$, respectively. For the example circuit, we have $U = (I \otimes U_2) (U_1 \otimes I) = U_{I2} U_{1I}$. The notation $U_{1I}$ refers to the unitary $(U_1 \otimes I)$, representing the Kronecker product of the $U_1$ operation with the identity operation on the remaining qubits (no operation can be represented as the identity operation). Similarly, $U_{I2}$ refers to the unitary $(I \otimes U_2)$. The post-synthesis approximations of these unitaries can be represented as $U' = (I \otimes U'_2) (U'_1 \otimes I) = U'_{I2} U'_{1I}$. Also, $N = N_I \times N_1 = N_2 \times N_I$.

As a first step, we prove the process distance bound when a unitary representing a partitioned block is extended to the remaining qubits in the full circuit, i.e., we determine the process distance of $U_1 \otimes I$ matrix given the process distance of the $U_1$ matrix. We begin by rearranging the terms in Eq.~\ref{eq:thames} to isolate for $\norm{\text{tr}(U^\dagger_1 U'_1)}$, as is shown in the derivation below.
\begin{equation}
    \begin{gathered}
        \sqrt{1 - \frac{\norm{\text{tr}(U^\dagger_1 U'_1)}^2}{N_1^2}} \le \epsilon_1 \\
        1 -\frac{\norm{\text{tr}(U^\dagger_1 U'_1)}^2}{N_1^2} \le \epsilon^2_1 \\
        \frac{\norm{\text{tr}(U^\dagger_1 U'_1)}^2}{N_1^2} \ge 1 - \epsilon^2_1 \\
        \norm{\text{tr}(U^\dagger_1 U'_1)}^2 \ge N_1^2(1 - \epsilon^2_1) \\
        \norm{\text{tr}(U^\dagger_1 U'_1)} \ge N_1\sqrt{1 - \epsilon^2_1}
    \end{gathered}
    \label{eq:nile}
\end{equation}

Next, we derive the relationship between $\text{tr}(U^\dagger_{1I}U'_{1I})$ and $\text{tr}(U^\dagger_1U'_1)$:
\begin{equation}
    \begin{gathered}
        \text{tr}(U^\dagger_{1I}U'_{1I}) = \text{tr}[(U_1 \otimes I)^\dagger(U'_1 \otimes I)] \\
         = \text{tr}[(U^\dagger_1 \otimes I^\dagger)(U'_1 \otimes I)] = \text{tr}[(U^\dagger_1 \otimes I)(U'_1 \otimes I)] \\
         = \text{tr}(U^\dagger_1U'_1 \otimes II) = \text{tr}(U^\dagger_1U'_1 \otimes I) \\
         = \text{tr}(U^\dagger_1U'_1)\text{tr(I)} = \text{tr}(U^\dagger_1U'_1)N_I
    \end{gathered}
    \label{eq:amazon}
\end{equation}

Substituting Eq.~\ref{eq:nile} into Eq.~\ref{eq:amazon}, we get that $\norm{\text{tr}(U^\dagger_{1I} U'_{1I})} \ge N\sqrt{1 - \epsilon^2_1}$, as shown below.
\begin{equation}
    \begin{gathered}
        \norm{\text{tr}(U^\dagger_{1I} U'_{1I})} = \norm{\text{tr}((U^\dagger_1U'_1)N_I} = \norm{\text{tr}((U^\dagger_1U'_1)}N_I \\
        \ge N_1\sqrt{1 - \epsilon^2_1}N_I = N_1 N_I\sqrt{1 - \epsilon^2_1} = N\sqrt{1 - \epsilon^2_1}
    \end{gathered}
    \label{eq:neponset}
\end{equation}

If we rearrange the terms in Eq.~\ref{eq:neponset} (similar to the rearranging in Eq.~\ref{eq:nile}, but in reverse order), we get $\sqrt{1 - \frac{\norm{\text{tr}(U^\dagger_{1I} U'_{1I})}^2}{N^2}} \le \epsilon_1$. Thus, the process distance of a block unitary that does not span the full size (number of qubits) of a circuit remains bounded by the same threshold when the unitary is extended to the size of the circuit. Therefore, using a similar procedure, we can also show that for the second block, $U_2$, $\sqrt{1 - \frac{\norm{\text{tr}(U^\dagger_{I2} U'_{I2})}^2}{N^2}} \le \epsilon_2$.

We now have the tools to bound the process distance of the full circuit $\bigg{(}\sqrt{1 - \frac{\norm{\text{tr}(U^\dagger U')}^2}{N^2}}\bigg{)}$. Substituting $U = U_{I2} U_{1I}$, we obtain the following:
\begin{equation}
    \begin{gathered}
    \sqrt{1 - \frac{\norm{\text{tr}(U^\dagger U')}^2}{N^2}} = \sqrt{1 - \frac{\norm{\text{tr}[(U_{I2} U_{1I})^\dagger(U'_{I2} U'_{1I})]}^2}{N^2}} \\
    = \sqrt{1 - \frac{\norm{\text{tr}(U^\dagger_{1I} U^\dagger_{I2} U'_{I2} U'_{1I})}^2}{N^2}} \\
    = \sqrt{1 - \frac{\norm{\text{tr}[(U'_{1I} U^\dagger_{1I})(U^\dagger_{I2} U'_{I2})]}^2}{N^2}}
    \end{gathered}
    \label{eq:hudson}
\end{equation}

Using the inequality proven by Wang and Zhang~\cite{wang1994trace} and using the above derived bounds for process distances of $U_{1I}$ and $U_{I2}$, the following relationship is obtained:

%\begin{equation}
\tiny
    \begin{gather}
    \sqrt{1 - \frac{\norm{\text{tr}[(U'_{1I} U^\dagger_{1I})(U^\dagger_{I2} U'_{I2})]}^2}{N^2}} \\
    \le \sqrt{1 - \frac{\norm{\text{tr}(U'_{1I} U^\dagger_{1I})}^2}{N^2}} + \sqrt{1 - \frac{\norm{\text{tr}(U^\dagger_2 U'_2)}^2}{N^2}} \\
    \le \sqrt{1 - \frac{\norm{\text{tr}(U^\dagger_{1I} U'_{1I})}^2}{N^2}} + \sqrt{1 - \frac{\norm{\text{tr}(U^\dagger_2 U'_2)}^2}{N^2}} \\
    \le \epsilon_{1I} + \epsilon_2
    \end{gather}
    \label{eq:danube}
%\end{equation}



Combining Eq.~\ref{eq:hudson} and Eq.~\ref{eq:danube}, we get $\sqrt{1 - \frac{\norm{\text{tr}(U^\dagger U')}^2}{N^2}} \le \epsilon_1 + \epsilon_2$. This proof can be extended to circuits partitioned into $K$ blocks by providing the proof for two blocks at a time, combining the two into a single unitary and providing the proof again for the two unitaries (combined unitary and the third unitary), and so on and so forth, iteratively. Therefore, for a circuit partitioned into $K$ blocks, we have that $\sqrt{1 - \frac{\norm{\text{tr}(U^\dagger U')}^2}{N^2}} \le \displaystyle\sum_{k=1}^{k=K}\epsilon_k$. Thus, the process distance of the full circuit is theoretically upper bounded by the sum of the process distances of all of its partitioned blocks. This derivation enables us to confidently bound the process distance of the full circuit simply by ensuring that its partitioned blocks are synthesized in a manner that the sum of their process distances is within an acceptable threshold. This method is linearly scalable in the number of partitioned block and eliminates the need to calculate the process distance of large full circuits, which is exponentially scalable in the number of qubits, and thus, infeasible to calculate for circuits with sizes beyond tens of qubits.







\red{\subsection{Generating Approximations}
  Partition. Enumerate sols. Reassemble. Pick target approx level and implement a procedure that minimizes depth and distance. Procedure not that important, here's ours.  Describe some algorithm..}



\subsection{\sol: Design and Implementation}

With the derivation of a tight theoretical upper bound, the next step is to employ a technique to make the best use of it. Recall that in Sec.~\ref{sec:background}, we demonstrated that the process distance does not have a one-to-one correlation with the final output distance obtained after executing the circuit and measuring the qubits. In fact, it is difficult to establish an analytical relationship between the process distance and the output distance. Two different circuits synthesized from the same original circuit that have similar process distances can have very different output distances. Therefore, simply choosing a synthesized circuit that has a process distance below a certain threshold and has a low depth does not guarantee that the output distance will also be minimal. To overcome this issue we propose \sol, a method to ensure that the output distance between the synthesized circuits and the original circuit is as low as possible without the need to calculate it directly.

The two parameters available to \sol{} for making the choice of synthesized circuits in a scalable manner are the upper bound of full circuit process distance (obtained as sum of process distances of circuit blocks) and the full circuit depth (or the number of CNOT gates -- the two parameters result in similar selection in most cases as the circuit depth is related to the number of CNOT gates it has). Therefore, as a first step, we can ensure that the synthesized circuit falls below a certain threshold $\epsilon$ in terms of the process distance upper bound calculated from block process distances. This step ensures that we filter out synthesizes circuits that are highly likely to have a large output distance. However, only considering synthesized circuits that are below a certain threshold still leaves us with multiple choices in terms of synthesized circuits and this is the key to reducing the output distance. Previous works have focused on finding the most optimal circuit (in terms of depth) that is below a certain threshold for actual process distance~\cite{}. In addition to this method being non-scalable due to requiring the calculation of actual process distance, it also does not consider the fact this most optimal circuit might still result in a relatively high output distance. Instead, we shift the focus to reducing the output distance without direct knowledge of it.

The key to achieving this reduction is realizing that multiple circuits can be synthesized such that they have process distance below a certain threshold. Recall that synthesis is performed using numerical optimization building layer-by-layer. What qubits these layers are placed on, what rotation angles are assigned to them, and how different blocks are put together to form the whole circuit affects the final synthesized circuit that is produced. Multiple synthesized circuits can be produced with upper bound process distance below a certain threshold can be produced by varying these factors. We discuss how \sol{} generates these circuits later in the section; however, first we demonstrate how they can be used to reduce the output distance. Fig.~\ref{fig:out_dist_cart} demonstrates a visual example of how selecting multiple synthesized circuits can help ensure that the output distance is reduced. Fig.~\ref{fig:out_dist_cart} (a) shows the output distance vs. circuit depth relationship of multiple synthesized circuits (all under the required upper bound process distance threshold). Fig.~\ref{fig:out_dist_cart} (b) shows the average output distance if $M$ circuits with the lowest depth are selected. If only the circuit with the minimum depth is selected, it can result in a high output distance. However, if more synthesized circuits are selected, we can reduce the output distance by averaging the results across all circuits.

Note that for some algorithms, the circuit with the lowest depth might also coincidentally have the one of the lower output distances. However, this can neither be established analytically, nor can it be established without calculating the output distance (which is non-scalable). Thus, averaging over $M$ low-depth circuits can help us regulate and control the output distance with more robustness than simply choosing one circuit with the lowest depth. The trade-off here is between the circuit depth and the output distance. If multiple circuits are not selected, we do not have a way to control, stabilize, and reduce the output error. On the other hand, if the depth becomes too high for a sub-section of the selected circuits, it can cause high-error on NISQ hardware. Therefore, we need to synthesize circuits in a manner that leaves us with multiple low-depth solutions that can be used to average the output distance for a more robust solution.

\begin{figure}[t]
    \centering
    \includegraphics[scale=0.3]{figures/end_to_end_cartoon.pdf}
    \caption{\sol's methodology of partitioning the circuit into smaller blocks, generating multiple solutions for each block, putting together blocks, and selecting the circuits with the lowest depths.}
    \label{fig:end_to_end_cart}
\end{figure}

To achieve this, we synthesis each circuit block to generate multiple synthesized versions. We modify the previously proposed LEAP compiler~\cite{} to generate circuit results at all acceptable depths. The LEAP compiler constructs a circuit tree one layer at a time. Each layer consists of a CNOT gate between two qubits followed by two three-axes rotation gates on both the qubits. It tries out this layer on all allowed two-qubit combinations and optimizes the rotation angles to minimize the unitary process distance. As more layers are added, the tree expands due to the increased number of layer permutations. Every few layers deep, the LEAP compiler pick the branch with the least process distance and starts reconstructing the tree from there to reduce the number of optimization evaluations. Finally, once the process distance becomes less than the required threshold for one of the branches, the compiler returns the corresponding synthesized circuit.

We modify this compiler to return the best $M$ circuits with the lowest process distance at each depth of the tree (tree depth roughly corresponds to circuit depth), once the process distance becomes less than a threshold. This allows us to generate different ``quality'' circuits (in terms of process distance) for each block at different depths. All solutions are returned until the tree exceeds the depth of the original circuit. As more layers are constructed and the tree becomes deeper, the process distance decreases as expected. However, because we would like to have multiple solutions for a block, including the ones with higher depth than the minimum depth solution, we collect all solutions of different depths. We also perform multiple compiler and numerical optimizer starts with different random seeds to capture more potential solutions for each block.

We perform this process for all blocks of a partitioned circuit. Note that the solutions for all blocks can be generated in parallel as the blocks are independent of each other by construction. After the completion of the process, it is time to put together all block solutions. Constructing the full circuits from the blocks simply requires appending the block circuits in the order of their original placement during partitioning. For a given synthesized full circuit, only one synthesized circuit can be used for each block. Thus, if there are 10 blocks, each with two synthesized circuit solutions, we can construct $2^10=1,024$ full synthesized circuits. Out of these circuits, we can select $M$ circuits with the lowest depths. Note that all full circuits will have lower upper bound process distance than the required threshold by construction. Full synthesized circuits that do not meet the threshold can be eliminated. \sol's methodology of generating multiple solutions for each block, putting together blocks, and selecting the circuits with the lowest depths is demonstrated in Fig.~\ref{fig:end_to_end_cart}. \sol{} provides a way to synthesize circuits in a manner that results in a low process distance, low circuit depth, and low output distance, without the need to directly calculate the full circuit process distance or output distance, thus, being the first solution that scales to large circuits.

In the next section, we evaluate the effectiveness of \sol{}, after providing details about the experimental setup and methodology.



